Electromagnetic cloak design with mono-objective and bi-objective optimizers: seeking the best tradeoff between protection and invisibility

We revisit the design of cloaks, without resorting to any geometric transform. Cancellation techniques and anomalous resonances have been applied for this purpose. Instead of a deductive reasoning, we propose a novel mono-objective optimization algorithm, namely a ternary grey wolf algorithm, and we adapt a bi-objective optimization algorithm. Firstly, the proposed chaotic ternary grey wolf algorithm searches three-valued spaces for all permittivity values in the cloak while minimizing the summation of a protection criterion and an invisibility criterion. Secondly, a bi-objective genetic algorithm is adapted to find pairs of optimal values of invisibility and protection.

==> NewCommands/TikzCommands.tex <==
\tikzstyle{decision} = [diamond, draw, fill=white, text centered, node distance=1cm, inner sep=0pt]

\tikzstyle{block} = [rectangle, draw, fill=yellow, text width=5em, text centered, node distance=1cm, minimum height=1em]

\tikzstyle{line} = [draw, -latex']

\tikzstyle{mycloud} = [cloud, draw,cloud puffs=10, cloud puff arc=120, aspect=2, text centered, text centered,fill=white, node distance=1cm, minimum height=2em]

\tikzstyle{Rect} = [rectangle, draw, fill=white, text width=5em, text centered, rounded corners, node distance=1cm, minimum height=4em]

\tikzstyle{InvisibleRectBlock} = [rectangle, fill=white, text width=5em, text centered,  node distance=3cm, minimum height=4em]

\tikzstyle{InvisibleCircleBlock} = [circle, fill=white, text width=5em, text centered, node distance=4cm, minimum height=2em]

\tikzstyle{CircleBlock} = [circle, draw, fill=white, text width=5em, text centered, node distance=4cm, minimum height=2em]

==> inputs/ApplicationInvisibility.tex <==

Problème à traiter :
Estimer trois valeurs entre 0 et 1, précisément 0.11, 0.22, et 0.33 symbolisant les valeurs de epsilon; ainsi que 64 valeurs de pixels dans l’espace de recherche $\left\{0,1,2\right\}$ . Ce sont donc plutôt des indices de valeurs, mais cela permet de reconstruire l’image.
Voici l’image cible à retrouver sans aucune connaissance a priori hormis la taille de l’image et le fait qu’il y a trois valeurs différentes, l'image estimée et les courbes de convergence pour trois méthodes dont celle proposée (monoobjectif).


\begin{figure}[h!]
\centering{
 \begin{tabular}{c@{\,}c@{\,}}
  \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Heavy_Setup8pixels/Expected.png} &
 \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Heavy_Setup8pixels/Estimated.png}\\
\includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Heavy_Setup8pixels/Three_Compared_Methods.png}&
   \end{tabular}
\caption{8 pixels; 200 agents, 50 iterations ; epsilon values: 0.09294329603029199, 0.22516238017368898, 0.33433604099442366; computational time 3 sec. \label{fig:HeavySetup8pixels} }}
\end{figure}


\begin{figure}[h!]
\centering{
 \begin{tabular}{c@{\,}c@{\,}}
  \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Light_Setup64pixels/Expected.png} &
 \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Light_Setup64pixels/Estimated.png}\\
\includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Light_Setup64pixels/Three_Compared_Methods.png}&
   \end{tabular}
\caption{64 pixels; 10 agents, 5 iterations; epsilon values:  '0.961513963853158', '0.30543607509286985', '0.0'.  computational time 0.2 sec. \label{fig:LightSetup64pixels} }}
\end{figure}

\begin{figure}[h!]
\centering{
 \begin{tabular}{c@{\,}c@{\,}}
  \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Heavy_Setup64pixels/Expected.png} &
 \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Heavy_Setup64pixels/Estimated.png}\\
\includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Heavy_Setup64pixels/Three_Compared_Methods.png}&
   \end{tabular}
\caption{64 pixels; 400 agents, 1000 iterations; epsilon values:  0.1099641609688962, 0.2200391529102906, 0.33002534069915285.  computational time 569 sec. Scores
GWO 1.532522712452121, GWO Discrete 1.3670784518623127, GWO continuous ternary binary 1.3355097906020004
\label{fig:HeavySetup64pixels} }}
\end{figure}

Scores corresponding to the results in Fig. \ref{fig:HeavySetup64pixels}:\\

\newpage

Test with L2 norm: 
\begin{figure}[h!]
\centering{
 \begin{tabular}{c@{\,}c@{\,}}
  \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Setup16pixels/Expected.png} &
 \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Setup16pixels/Estimated.png}\\
\includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Setup16pixels/Three_Compared_Methods.png}&
   \end{tabular}
\caption{16 pixels; 500 agents, 50 iterations; epsilon values: 0.111374306635323, 0.2208907850873558, 0.33139529971003606.  computational time ~20 sec. Scores GWO 0.005842013525459382, GWO Discrete 0.01821568901058088,
GWO continuous ternary binary 8.847989184417474e-05
\label{fig:16pixels}}}
\end{figure}

\newpage

Test light setup et interpolation: 
\begin{figure}[h!]
\centering{
 \begin{tabular}{c@{\,}c@{\,}}
  \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Setup_64_Pixels_Interpolation/Expected.png} &
 \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Setup_64_Pixels_Interpolation/EstimatedSmall.png}\\
 \includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Setup_64_Pixels_Interpolation/Estimated.png}&
\includegraphics[width=4.0cm]{Figures/ApplicationInvisibility/Setup_64_Pixels_Interpolation/Three_Compared_Methods.png}
   \end{tabular}
\caption{64 pixels; interpolation; 80 agents, 50 iterations; expected epsilon values:0.22 0.71 0.66; estimated epsilon values 0.22188605 0.70932152 0.66426907.  computational time ~7 sec. Scores: GWO 0.016791808735886322, GWO Discrete 0.020625308628104553, GWO continuous ternary binary 0.0002718003690306721\label{fig:64pixelsinterpolation}}}
\end{figure}

\newpage


==> inputs/ApplicationOptimisationOld.tex <==
%L'objectif est d'optimiser une cape d'invisibilité en forme d'un demi rectangle.

%Nous avons appliqué un maillage triangulaire sur cette cape, et cette dernière se retrouve être constituée de 329 mailles, ou triangles.

%L'optimisation en question consiste à minimiser les deux critères qui sont l'invisibilité et la protection, tels que nous avons défini ces critères au paragraphe 3.3.

%Pour y parvenir, l'idée est d'attribuer les "meilleures" valeurs d'epsilon possible pour chacun des triangles.

The objective is to optimize an invisibility cloak in the shape of a half rectangle.

We have applied a triangular mesh on this cloak, and it is made of 329 meshes, or triangles.

The optimization in question consists in minimizing the two criteria which are invisibility and protection, as we defined these criteria in paragraph 3.3.

To achieve this, the idea is to assign the "best" possible epsilon values for each of the triangles.

\subsection{Mono-objective approach:}\label{subsec:monoobjectiveapproach}

%Dans un premier temps, pour rester dans le domaine du possible, nous avons limité à trois le nombre de valeurs d'epsilon possibles (pour chacun des triangles).

%Dans la mesure où l'optimisation topologique limite à deux le nombre de valeurs possibles, nous avons choisi des méthodes d'optimisation qui permettent de travailler sur un espace de recherche ayant plus de deux valeurs.

%Ainsi, on a donc indexé avec les indices : '0', '1' et '2', tois valeurs d'epsilon choisies arbitrairement, soient, respectivement, '7', '10', et '12'.

%On a commencé nos tests avec trois variantes d'une méthode mono-objectif d'optimisation bio-inspirée : la méthode dite du "loup gris", ou Grey Wolf Optimization (GWO).

%La première variante, ou méthode de référence, est la méthode du "loup gris" (GWO), dans sa version originale.

%La deuxième variante, que nous avons nommé "GWO Discrete", consiste à ne travailler qu'avec des valeurs entières, en l'occurrence '0', '1', et '2' pour que cela soit consistant avec les valeurs de nos indices, et cela, sans toutefois utiliser une fonction pour arrondir les valeurs obtenues en valeurs entières. En effet, la particularité de cette variante est d'utiliser une "power map", tel que cela est présenté en Fig. 1, c'est-à-dire une superficie que nous divisons en trois zones ('0', '1', et '2'), puis, en considérant : la valeur obtenue comme position sur l'axe horizontal, et une valeur tirée aléatoirement comme position sur l'axe vertical, on obtient un point dans une des trois zones de cette superficie. Bien entendu, le découpage en trois zones, de la superficie, n'est pas aléatoire : on attribue une grande superficie à la zone '0' quand on est proche du "zéro" sur l'axe horizontal, on attribue une grande superficie à la zone '1' quand on est proche du "un" sur l'axe horizontal, et on attribue une grande superficie à la zone '2' quand on est proche de la valeur "deux" sur l'axe horizontal. Malgré tout, on conserve une petite probabilité pour que le numéro de la zone dans laquelle on va se placer ne corresponde pas à la valeur obtenue, utilisée comme position sur l'axe horizontal. L'intérêt d'une telle discordance est d'éviter à notre algorithme de se laisser enfermer dans un minimum local.

Initially, in order to remain in the realm of the possible, we limited the number of possible epsilon values to three (for each of the triangles).

Since topological optimization limits the number of possible values to two, we have chosen optimization methods that allow us to work on a search space with more than two values.

Thus, we indexed with the indices: '0', '1' and '2', three arbitrarily chosen values of epsilon, that is, respectively, '7', '10', and '12'.

We started our tests with three variants of a single-objective bio-inspired optimization method: the so-called Grey Wolf Optimization (GWO) method.

The first variant, or reference method, is the Grey Wolf Optimization (GWO) method, in its original version.

The second variant, which we have named "GWO Discrete", consists in working only with integer values, in this case '0', '1', and '2', so that it is consistent with the values of our indices, and this, without using a function to round the values obtained in integer values. Indeed, the particularity of this variant is to use a "power map", as it is presented in Fig. 1, i.e. an area that we divide into three zones ('0', '1', and '2'), then, considering: the value obtained as a position on the horizontal axis, and a randomly drawn value as a position on the vertical axis, we obtain a point in one of the three zones of this area. Of course, the division of the area into three zones is not random: a large area is attributed to zone '0' when it is close to "zero" on the horizontal axis, a large area is attributed to zone '1' when it is close to "one" on the horizontal axis, and a large area is attributed to zone '2' when it is close to the value "two" on the horizontal axis. Nevertheless, there is still a small probability that the number of the area in which we are going to place ourselves does not correspond to the value obtained, used as a position on the horizontal axis. The interest of such a mismatch is to avoid our algorithm to be locked in a local minimum.

%Enfin, la troisième variante, que nous avons nommé "Chaotic Binary Ternary Grey Wolf Optimization", reprend le principe de la "power map" pour un espace de recherche à deux ou trois valeurs, et introduit également une séquence chaotique dans l'algorithme de recherche du minimum global. Là encore, la séquence chaotique a pour intérêt d'éviter un enfermement dans un minimum local.

%Rappelons également que nous avons deux critères à minimiser alors que nous utilisons les variantes d'une méthode d'optimisation qui est mono-objectif... Autrement dit, c'est la somme de nos deux critères qui constitue notre objectif, et que nous minimisons.

%Voici donc les résultats que nous avons ainsi obtenus pour chacune de ces trois méthodes.

Finally, the third variant, which we have named "Chaotic Ternary Grey Wolf Optimization", takes up the principle of the "power map" for a search space with two or three values, and also introduces a chaotic sequence in the algorithm for finding the global minimum. Here again, the chaotic sequence has the advantage of avoiding a confinement in a local minimum.

Let us also recall that we have two criteria to minimize while we are using variants of an optimization method which is mono-objective... In other words, it is the sum of our two criteria that constitutes our objective, and that we minimize.

Here are the results we obtained for each of these three methods.

\newpage

\subsubsection{Case number one: Mono-objective optimization, 250 iterations, 100 agents}\label{subsubsec:resmonoobjectif}
\paragraph{Results}
\begin{figure*}[h!]
    \centering{
        \begin{tabular}{c@{\,}c@{\,}}
             Cloak design & Wave propagation field\\
            \includegraphics[width=0.49\linewidth]{./Figures/cas1/50-50 GWO.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas1/Methode 1.JPG}\\
         (a) & (d) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas1/50-50 Discrete GWO.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas1/Methode 2.JPG}\\
         (b) & (e) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas1/50-50 CBTGWO.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas1/Methode 3.JPG}\\
         (c) & (f) \\
        \end{tabular}
        \caption{Row 1: in (a) GWO optimized cloak, in (b) Discrete GWO optimized cloak, and in (c), CTGWO optimized cloak; Row 2: in (d) GWO result, in (e) Discrete GWO result, and in (f), CTGWO result  \label{fig:f5}}}
\end{figure*} 

\paragraph{Convergence curves} 
\begin{figure*}[h!]
	\centering{
		\includegraphics[scale=0.6]{Figures/Optimization/Mi-cape Three_Compared_Methods.png} %Three_Compared_Methods.png}
		\caption{ Convergence curve of CTGWO, GWO and amixedGWO algorithms }}
\end{figure*}
\paragraph{Numerical results}
\begin{table*}[h!]
	\centering
	\resizebox{1.10\textwidth}{!}{
\begin{tabular}{cc|ccc}
\hline
\multicolumn{2}{c}{Cas} & GWO & amixedGWO & CTGWO\\
\hline
$Half-rectangle$& Protection&0.0042343101366780255&0.0003481234829584469&0.00015608238359645862\\
$100-agents$& Invisibility&0.0017399327049968023&0.0009572061288221007&0.0008695749972742106\\
$250-iterations$& Mean&0.002987121420837414&0.0006526648058902739&0.0005128286904353347\\
 & Links to figures& fig. \ref{fig:f5}(d)& fig. \ref{fig:f5}(e)& fig. \ref{fig:f5}(f)\\
			\hline
		\end{tabular}
	}
	\caption{Comparison of GWO, amixedGWO and CTGWO mono-objective methods in protection and invisibility for a rectangular and half-rectangular cape.}\label{Table:labeldecadixadesyeuxdevelours}
\end{table*}
%Comparaison des methodes mono-objectif GWO, amixedGWO et CTGWO en protection et en invisibilite pour une cape rectangulaire et demi-rectangulaire.


\subsection{Bi-objective approach:}\label{subsec:biobjectiveapproach}

%Dans un deuxième temps, nous avons utilisé un algorithme génétique bi-objectif comme méthode d'optimisation.

%La particularité de l'approche bi-objectif est que l'optimisation se fait sur les deux critères en même temps, tel que cela a été détaillé dans le paragraphe 2.2.

%Ainsi, nous ne travaillons plus sur des courbes de convergence, mais sur des fronts de Pareto.

In a second step, we used a bi-objective genetic algorithm as an optimization method.

The particularity of the bi-objective approach is that the optimization is done on both criteria at the same time, as detailed in paragraph 2.2.

Thus, we no longer work on convergence curves, but on Pareto fronts.

%, c'est-à-dire qu'une solution est considérée comme étant meilleure qu'une autre solution si elle est meilleure dans un des deux critères et qu'elle est meilleure ou égale dans l'autre critère. On appelle ce principe la "domination".

%Autrement dit, si on considère la valeur d'une solution pour un premier critère, représenté sur l'axe des X, et la valeur de cette même solution mais dans le second critère, représenté, lui, sur l'axe des Y, alors pour chaque solution, on va considérer sa distance avec le point d'origine (de coordonnées (0,0)). Plus cette distance sera courte, et meilleure sera la solution.

%Pour trier les meilleures solutions, il existe également une autre approche, qui, par opposition au principe de "domination" s'appelle la "non-domination". Cette méthode est assez complexe, mais pour faire simple on dira qu'on ne considère plus la distance par rapport à l'origine mais une distance dite "d'encombrement" qui se calcule en additionnant la valeur en X avec la valeur en Y. En utilisant ce système de mesure, certaines solutions qui auraient été écartées parce que leurs distances par rapport à l'origine auraient été trop grandes, sont remises en compétition.

%Dans la littérature, il est dit que la méthode d'optimisation bi-objectif Non-dominated Sorted Genetic Algorithm - II (NSGA-II) est une des méthodes parmi les plus efficaces, c'est pourquoi nous avons choisi d'utiliser cette méthode.

%C'est donc toujours avec nos trois valeurs d'epsilon '7', '10', et '12', indexées en '0', '1', et '2', mais en utilisant cette fois une méthode d'optimisation bi-objectif, en l'occurrence le NSGA-II, que nous avons procédé à deux optimisations : la première avec 250 itérations et 100 agents, la seconde avec 1000 itérations et 200 agents.

%Voici donc les résultats que nous avons obtenus.

So, it is still with our three epsilon values '7', '10', and '12', indexed in '0', '1', and '2', but using this time a bi-objective optimization method, in this case the NSGA-II, that we proceeded to two optimizations: the first one with 250 iterations and 100 agents, the second one with 1000 iterations and 200 agents.

Here are the results we obtained.

\newpage
\subsubsection{Case number two: Bi-objective ternary optimization with 250 iterations, 100 research agents.}
\paragraph{Results}
\begin{figure*}[h!]
    \centering{
        \begin{tabular}{c@{\,}c@{\,}}
             Cloak design & Wave propagation field\\
            \includegraphics[width=0.49\linewidth]{./Figures/cas2/invis_cape_gen.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas2/invis_genetic_norm.jpg}\\
         (a) & (d) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas2/mean2_cape_gen.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas2/mean2_genetic_norm.jpg}\\
         (b) & (e) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas2/protec_cape_gen.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas2/protec_genetic_norm.jpg}\\
         (c) & (f) \\
        \end{tabular}
        \caption{ Row 1: in (a) Best invisibility cloak, in (b) Best compromise between invisibility and protection cloak, and in (c), Best protection cloak; Row 2: in (d) Best invisibility result, in (e) Best compromise between invisibility and protection result, and in (f), Best protection result. \label{fig:f7}}}
\end{figure*}
\paragraph{Pareto front}
\begin{figure}[H]
	\centering{
			\includegraphics[scale=0.45]{Figures/Optimization/Front de pareto code genetique+zoom - 250 ite.png}

		\caption{ In red, the four selected solutions.}}
\end{figure}
\paragraph{Numerical results}
\begin{center}
	\begin{table*}[h!]
		\centering{
			\begin{tabular}{cc|ccc}
				\hline
				\multicolumn{2}{c}{Case} & Protection & Invisibility & Link to figure\\
				\hline
$Half-rectangle$& Best Protection&0.00016903308539718457&0.0008922496715084679&fig. \ref{fig:f7}(f)\\
$100-agents$& Best Invisibility&0.0010765244967287531&0.0005362717180578936&fig. \ref{fig:f7}(d)\\
$250-iterations$& Best Mean&0.00046434484599299766&0.000652728258292644&fig. \ref{fig:f7}(e)\\
\hline
        	\end{tabular}
			\caption{Comparison of a NSGA-II bi-objective method in protection and invisibility for a half-rectangular cloak. \label{Table:labeldecadixadesyeuxdevelours2} }}
	\end{table*}
\end{center}
\subsubsection{Case number two: Bi-objective ternary optimization with 1000 iterations, 200 research agents.}
\paragraph{Results}
\begin{figure*}[h!]
    \centering{
        \begin{tabular}{c@{\,}c@{\,}}
             Cloak design & Wave propagation field\\
            \includegraphics[width=0.49\linewidth]{./Figures/cas2/1000invis_capegen_sou.jpg} &\includegraphics[width=0.49\linewidth]{./Figures/cas2/1000invis_genetic_norm_source2.jpg}\\
         (a) & (d) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas2/1000mean2_cape_gen_so.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas2/1000mean2_genetic_norm_source2.jpg}\\
         (b) & (e) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas2/1000protec_cape_gen_s.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas2/1000protec_genetic_norm_source2.jpg}\\
         (c) & (f) \\
        \end{tabular}
        \caption{ Row 1: in (a) Best invisibility cloak, in (b) Best compromise between invisibility and protection cloak, and in (c), Best protection cloak; Row 2: in (d) Best invisibility result, in (e) Best compromise between invisibility and protection result, and in (f), Best protection result. \label{fig:f9}}}
\end{figure*}
\paragraph{Pareto front}
\begin{figure}[h!]
	\centering{
			\includegraphics[scale=0.8]{Figures/Optimization/1000pareto_source2.jpg}

		\caption{ In red, the four selected solutions out of a total of 175 }}
\end{figure}
\paragraph{Numerical results}
\begin{center}
	\begin{table*}[h!]
		\centering{
			\begin{tabular}{cc|ccc}
				\hline
				\multicolumn{2}{c}{Case} & Protection & Invisibility & Link to figure\\
\hline
$Half-rectangle$& Best Protection&0.0001233556779295822&0.0006808233349312879&fig. \ref{fig:f9}(f)\\
$200-agents$& Best Invisibility&0.001006414416092534&0.00043123852989015136&fig. \ref{fig:f9}(d)\\
$1000-iterations$& Best Mean&0.00040597975114207725&0.0005198314758624204&fig. \ref{fig:f9}(e)\\
				\hline
			\end{tabular}
			\caption{Comparison of a NSGA-II bi-objective method in protection and invisibility for a half-rectangular cloak. \label{Table:labeldecadixadesyeuxdevelours2} }}
	\end{table*}
\end{center}

Here are the results we obtained.

\newpage

\subsubsection{Case number three: Bi-objective continuous optimization with 250 iterations, 100 research agents.}
\paragraph{Results}
\begin{figure*}[h!]
    \centering{
        \begin{tabular}{c@{\,}c@{\,}}
             Cloak design & Wave propagation field\\
            \includegraphics[width=0.49\linewidth]{./Figures/cas3/BEST_Invisibility_cloak.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas3/BEST_Invisibility_field.jpg}\\
         (a) & (d) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas3/BEST_Mean_cloak.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas3/BEST_Mean_field.jpg}\\
         (b) & (e) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas3/BEST_Protect_cloak.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas3/BEST_Protect_field.jpg}\\
         (c) & (f) \\
        \end{tabular}
        \caption{ Row 1: in (a) Best invisibility cloak, in (b) Best compromise between invisibility and protection cloak, and in (c), Best protection cloak; Row 2: in (d) Best invisibility result, in (e) Best compromise between invisibility and protection result, and in (f), Best protection result. \label{fig:f11}}}
\end{figure*}
\paragraph{Pareto front}
\begin{figure}[h!]
	\centering{
			\includegraphics[scale=0.45]{Figures/Optimization/Pareto av zoom.png}

		\caption{ In red, the four selected solutions.}}
\end{figure}
\paragraph{Numerical results}
\begin{center}
	\begin{table*}[h!]
		\centering{
			\begin{tabular}{cc|ccc}
				\hline
				\multicolumn{2}{c}{Case} & Protection & Invisibility & Link to figure\\
				\hline
$Half-rectangle$& Best Protection&0.00007845140595910772&0.0004302410353088411&fig. \ref{fig:f11}(f)\\
$100-agents$& Best Invisibility&0.00044190355957334074&0.000032741951781281986&fig. \ref{fig:f11}(d)\\
$250-iterations$& Best Mean&0.00016660076580053048&0.00011668570132422142&fig. \ref{fig:f11}(e)\\
				\hline
			\end{tabular}
			\caption{Comparison of a NSGA-II bi-objective method in protection and invisibility for a half-rectangular cloak. \label{Table:labeldecadixadesyeuxdevelours2} }}
	\end{table*}
\end{center}
\subsubsection{Case number three: Bi-objective continuous optimization with 1000 iterations, 200 research agents.}
\paragraph{Results}
\begin{figure*}[h!]
    \centering{
        \begin{tabular}{c@{\,}c@{\,}}
             Cloak design & Wave propagation field\\
            \includegraphics[width=0.49\linewidth]{./Figures/cas3/1000BEST_Invis_cloak.jpg} &\includegraphics[width=0.49\linewidth]{./Figures/cas3/1000BEST_Invis_field.jpg}\\
         (a) & (d) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas3/1000BEST_Mean_cloak.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas3/1000BEST_Mean_field.jpg}\\
         (b) & (e) \\
        \includegraphics[width=0.49\linewidth]{./Figures/cas3/1000BEST_Protect_cloak.jpg}    &\includegraphics[width=0.49\linewidth]{./Figures/cas3/1000BEST_Protect_field.jpg}\\
         (c) & (f) \\
        \end{tabular}
        \caption{ Row 1: in (a) Best invisibility cloak, in (b) Best compromise between invisibility and protection cloak, and in (c), Best protection cloak; Row 2: in (d) Best invisibility result, in (e) Best compromise between invisibility and protection result, and in (f), Best protection result. \label{fig:f13}}}
\end{figure*}
\paragraph{Pareto front}
\begin{figure}[h!]
	\centering{
			\includegraphics[scale=0.45]{Figures/Optimization/Pareto2 avec zoom.png}

		\caption{ In red, the four selected solutions.}}
\end{figure}
\paragraph{Numerical results}
\begin{center}
	\begin{table*}[h!]
		\centering{
			\begin{tabular}{cc|ccc}
				\hline
				\multicolumn{2}{c}{Case} & Protection & Invisibility & Link to figure\\
				\hline
$Half-rectangle$& Best Protection&0.00006305848490381322&0.00023408700901736073&fig. \ref{fig:f13}(f)\\
$200-agents$& Best Invisibility&0.0007782354112551082&0.000025917328991204385&fig. \ref{fig:f13}(d)\\
$1000-iterations$& Best Mean&0.0001529618980280156&0.00006740873459052437&fig. \ref{fig:f13}(e)\\
\hline
			\end{tabular}
			\caption{Comparison of a NSGA-II bi-objective method in protection and invisibility for a half-rectangular cloak. \label{Table:labeldecadixadesyeuxdevelours2} }}
	\end{table*}
\end{center}


==> inputs/CodeTikzOther.tex <==



\begin{figure}[h!]
\centering
\begin{tikzpicture}[x=2.9cm,y=1.0cm]
  \readlist\Nnod{7,3,5} % array of number of nodes per layer
  \readlist\Nstr{N,L,M} % array of string number of nodes per layer
  \readlist\Cstr{I,Z,O} % array of coefficient symbol per layer
  \def\yshift{0.55} % shift last node for dots
  
  % LOOP over LAYERS
  \foreachitem \N \in \Nnod{
    \def\lay{\Ncnt} % alias of index of current layer
    \pgfmathsetmacro\prev{int(\Ncnt-1)} % number of previous layer
    \foreach \i [evaluate={\c=int(\i==\N); \y=\N/2-\i-\c*\yshift;
                 \x=\lay; \n=\nstyle;
                 \index=(\i<\N?int(\i):"\Nstr[\n]");}] in {1,...,\N}{ % loop over nodes
      % NODES
      \node[node \n] (N\lay-\i) at (\x,\y) {$\strut\Cstr[\n]_{\index}$};
      
      % CONNECTIONS
      \ifnumcomp{\lay}{>}{1}{ % connect to previous layer
        \foreach \j in {1,...,\Nnod[\prev]}{ % loop over nodes in previous layer
          \draw[white,line width=0.8,shorten >=1] (N\prev-\j) -- (N\lay-\i);
          \draw[connect] (N\prev-\j) -- (N\lay-\i);
        }
        \ifnum \lay=\Nnodlen
          \draw[connect] (N\lay-\i) --++ (0.5,0); % arrows out
        \fi
      }{
        \draw[connect] (0.5,\y) -- (N\lay-\i); % arrows in
      }
      
    }
    \path (N\lay-\N) --++ (0,1+\yshift) node[midway,scale=1.6] {$\vdots$}; % dots
  }
  
  % LABELS
  \node[above=0.5,align=center,mydarkgreen] at (N1-1.90) {Input\\[-0.2em]layer};
  \node[above=2.5,align=center,mydarkblue] at (N2-1.90) {Hidden\\[-0.2em]layer};
    \node[above=0.5,align=center,mydarkblue] at (N2-1.90) {~\\[-0.2em]~};
  \node[above=1.5,align=center,mydarkred] at (N\Nnodlen-1.90) {Output\\[-0.2em]layer};
  
\end{tikzpicture}
  \caption{General scheme for an Artificial Neural Network.\label{fig:schema-ANN}}
\end{figure}







\begin{tikzpicture}[
    shorten >=1pt, shorten <=1pt,
    neuron/.style={circle, draw, minimum size=4ex, thick},
    legend/.style={font=\large\bfseries},
  ]
  % encoder
  \drawNodes{encoder}{{{,,,,}, {,,,}, {,,}}}
  \denselyConnectNodes{encoder}{{5, 4, 3}}

  % decoder
  \begin{scope}[xshift=11cm]
    \drawNodes{decoder}{{{,,}, {,,,}, {,,,,}}}
    \denselyConnectNodes{decoder}{{3, 4, 5}}
  \end{scope}

  % mu, sigma, sample nodes
  \foreach \idx in {1,...,3} {
      \coordinate[neuron, right=2 of encoder-3-2, yshift=\idx cm,, fill=yellow, fill opacity=0.2] (mu-\idx);
      \coordinate[neuron, right=2 of encoder-3-2, yshift=-\idx cm, fill=blue, fill opacity=0.1] (sigma-\idx);
      \coordinate[neuron, right=4 of encoder-3-2, yshift=\idx cm-2cm, fill=green, fill opacity=0.1] (sample-\idx);
    }

  % mu, sigma, sample boxes
  \node [label=$\mu$, fit=(mu-1) (mu-3), draw, fill=yellow, opacity=0.45] (mu) {};
  \node [label=$\sigma$, fit=(sigma-1) (sigma-3), draw, fill=blue, opacity=0.3] (sigma) {};
  \node [label=sample, fit=(sample-1) (sample-3), draw, fill=green, opacity=0.3] (sample) {};

  % mu, sigma, sample connections
  \draw[->] (mu.east) edge (sample.west) (sigma.east) -- (sample.west);
  \foreach \a in {1,2,3}
  \foreach \b in {1,2,3} {
      \draw[->] (encoder-3-\a) -- (mu-\b);
      \draw[->] (encoder-3-\a) -- (sigma-\b);
      \draw[->] (sample-\a) -- (decoder-1-\b);
    }

  % input + output labels
  \foreach \idx in {1,...,5} {
      \node[left=0 of encoder-1-\idx] {$x_\idx$};
      \node[right=0 of decoder-3-\idx] {$\hat x_\idx$};
    }
  \node[above=0.1 of encoder-1-1] {input};
  \node[above=0.1 of decoder-3-1] {output};

\end{tikzpicture}


% NEURAL NETWORK activation
% https://www.youtube.com/watch?v=aircAruvnKk&list=PLZHQObOWTQDNU6R1_67000Dx_ZCJB-3pi&index=1
\begin{tikzpicture}[x=2.7cm,y=1.6cm]
  \message{^^JNeural network activation}
  \def\NI{5} % number of nodes in input layers
  \def\NO{4} % number of nodes in output layers
  \def\yshift{0.4} % shift last node for dots
  
  % INPUT LAYER
  \foreach \i [evaluate={\c=int(\i==\NI); \y=\NI/2-\i-\c*\yshift; \index=(\i<\NI?int(\i):"n");}]
              in {1,...,\NI}{ % loop over nodes
    \node[node in,outer sep=0.6] (NI-\i) at (0,\y) {$a_{\index}^{(0)}$};
  }
  
  % OUTPUT LAYER
  \foreach \i [evaluate={\c=int(\i==\NO); \y=\NO/2-\i-\c*\yshift; \index=(\i<\NO?int(\i):"m");}]
    in {\NO,...,1}{ % loop over nodes
    \ifnum\i=1 % high-lighted node
      \node[node hidden]
        (NO-\i) at (1,\y) {$a_{\index}^{(1)}$};
      \foreach \j [evaluate={\index=(\j<\NI?int(\j):"n");}] in {1,...,\NI}{ % loop over nodes in previous layer
        \draw[connect,line width=1.2] (NI-\j) -- (NO-\i);%white,
        \draw[connect] (NI-\j) -- (NO-\i)
          node[pos=0.50] {{$w_{1,\index}$}};%\contour{white}
      }
    \else % other light-colored nodes
      \node[node,blue!20!black!80,draw=myblue!20,fill=myblue!5]
        (NO-\i) at (1,\y) {$a_{\index}^{(1)}$};
      \foreach \j in {1,...,\NI}{ % loop over nodes in previous layer
        %\draw[connect,white,line width=1.2] (NI-\j) -- (NO-\i);
        \draw[connect,myblue!20] (NI-\j) -- (NO-\i);
      }
    \fi
  }
  
  % DOTS
  \path (NI-\NI) --++ (0,1+\yshift) node[midway,scale=1.2] {$\vdots$};
  \path (NO-\NO) --++ (0,1+\yshift) node[midway,scale=1.2] {$\vdots$};
  
  % EQUATIONS
  \def\agr#1{{\color{mydarkgreen}a_{#1}^{(0)}}}
  \node[below=17,right=11,mydarkblue,scale=0.95] at (NO-1)
    {$\begin{aligned} %\underset{\text{bias}}{b_1}
       &= \color{mydarkred}\sigma\left( \color{black}
            w_{1,0}\agr{0} + w_{1,1}\agr{1} + \ldots + w_{1,n}\agr{n} + b_1^{(0)}
          \color{mydarkred}\right)\\
       &= \color{mydarkred}\sigma\left( \color{black}
            \sum_{i=1}^{n} w_{1,i}\agr{i} + b_1^{(0)}
           \color{mydarkred}\right)
     \end{aligned}$};
  \node[right,scale=0.9] at (1.3,-1.3)
    {$\begin{aligned}
      {\color{mydarkblue}
      \begin{pmatrix}
        a_{1}^{(1)} \\[0.3em]
        a_{2}^{(1)} \\
        \vdots \\
        a_{m}^{(1)}
      \end{pmatrix}}
      &=
      \color{mydarkred}\sigma\left[ \color{black}
      \begin{pmatrix}
        w_{1,0} & w_{1,1} & \ldots & w_{1,n} \\
        w_{2,0} & w_{2,1} & \ldots & w_{2,n} \\
        \vdots  & \vdots  & \ddots & \vdots  \\
        w_{m,0} & w_{m,1} & \ldots & w_{m,n}
      \end{pmatrix}
      {\color{mydarkgreen}
      \begin{pmatrix}
        a_{1}^{(0)} \\[0.3em]
        a_{2}^{(0)} \\
        \vdots \\
        a_{n}^{(0)}
      \end{pmatrix}}
      +
      \begin{pmatrix}
        b_{1}^{(0)} \\[0.3em]
        b_{2}^{(0)} \\
        \vdots \\
        b_{m}^{(0)}
      \end{pmatrix}
      \color{mydarkred}\right]\\[0.5em]
      {\color{mydarkblue}a^{(1)}}
      &= \color{mydarkred}\sigma\left( \color{black}
           \mathbf{W}^{(0)} {\color{mydarkgreen}a^{(0)}}+\mathbf{b}^{(0)}
         \color{mydarkred}\right)
         %\color{black},\quad \mathbf{W}^{(0)} \in \mathbb{R}^{m\times n}
    \end{aligned}$};
  
\end{tikzpicture}


\begin{neuralnetwork}[height=8]
  \tikzstyle{input neuron}=[neuron, fill=orange!70];
  \tikzstyle{output neuron}=[neuron, fill=blue!60!black, text=white];

  \inputlayer[count=8, bias=false, title=Input Layer, text=\xin]

  \hiddenlayer[count=5, bias=false]
  \linklayers

  \hiddenlayer[count=3, bias=false, title=Latent\\Representation]
  \linklayers

  \hiddenlayer[count=5, bias=false]
  \linklayers

  \outputlayer[count=8, title=Output Layer, text=\xout]
  \linklayers

\end{neuralnetwork}


%%%%


\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \node (x) at (0.5,0) {$x$};
    \node[fc] (fc1) at (2,0) {\small$\text{fc}_{C_0, C_1}$};
    \node[bias] (b1) at (3.5,0) {\small$\text{bias}$};
    \node[h] (h1) at (4.5,0) {\small$h$};
    \node[fc] (fc2) at (5.75,0) {\small$\text{fc}_{C_1, C_2}$};
    \node[bias] (b2) at (7.25,0) {\small$\text{bias}$};
    \node[h] (h2) at (8.25,0) {\small$h$};
    \node[fc] (fc3) at (9.5,0) {\small$\text{fc}_{C_2, C_3}$};
    \node[bias] (b3) at (11,0) {\small$\text{bias}$};
    \node[h] (h3) at (12,0) {\small$h$};
    \node (y) at (13.5,0) {\small$y$};
    \draw[->] (x) -- (fc1);
    \draw[->] (fc1) -- (b1);
    \draw[->] (b1) -- (h1);
    \draw[->] (h1) -- (fc2);
    \draw[->] (fc2) -- (b2);
    \draw[->] (b2) -- (h2);
    \draw[->] (h2) -- (fc3);
    \draw[->] (fc3) -- (b3);
    \draw[->] (b3) -- (h3);
    \draw[->] (h3) -- (y);
  \end{tikzpicture}
  \vskip 6px
  % TODO short caption
  % TODO parameters
  \caption[]{Illustration of a multi-layer perceptron with $L = 3$ fully-connected 
  layers followed by bias layers and non-linearities. The sizes $C_1$ and $C_2$ are
  hyper-parameters while $C_0$ and $C_3$ are determined by the problem at hand.
Overall, the multi-layer perceptron represents a function $y(x;w)$ parameterized by
the weights $w$ in the fully-connected and bias layers.}
  \label{fig:deep-learning-mlp}
\end{figure}

\begin{figure}
  \centering
  \begin{tikzpicture}
    \node (x) at (1.25,0) {\small$x$};
  
    \node[fc,rotate=90,minimum width=2cm] (fc1) at (2.5,0) {\small$\text{fc}_{R, C_1}$};
    \node[bias,rotate=90,minimum width=2cm] (b1) at (3.75,0) {\small$\text{bias}$};
    \node[h,rotate=90,minimum width=2cm] (h1) at (5,0) {\small$h$};
    \node[fc,rotate=90,minimum width=2cm] (fc2) at (6.25,0) {\small$\text{fc}_{C_1, C_2}$};
    \node[bias,rotate=90,minimum width=2cm] (b2) at (7.5,0) {\small$\text{bias}$};
    \node[h,rotate=90,minimum width=2cm] (h2) at (8.75,0) {\small$h$};
    \node[fc,rotate=90,minimum width=2cm] (fc3) at (10,0) {\small$\text{fc}_{C_2, Q}$};
    \node[bias,rotate=90,minimum width=2cm] (b3) at (11.25,0) {\small$\text{bias}$};
    \node[h,rotate=90,minimum width=2cm] (h3) at (12.5,0) {\small$h$};
  
    \node (z) at (13.75,-2.5) {\small$z$};
  
    \node[h,rotate=90,minimum width=2cm] (h6) at (2.5,-2.5) {\small$h$};
    \node[bias,rotate=90,minimum width=2cm] (b6) at (3.75,-2.5) {\small$\text{bias}$};
    \node[fc,rotate=90,minimum width=2cm] (fc6) at (5,-2.5) {\small$\text{fc}_{C_1, R}$};
    \node[h,rotate=90,minimum width=2cm] (h5) at (6.25,-2.5) {\small$h$};
    \node[bias,rotate=90,minimum width=2cm] (b5) at (7.5,-2.5) {\small$\text{bias}$};
    \node[fc,rotate=90,minimum width=2cm] (fc5) at (8.75,-2.5) {\small$\text{fc}_{C_2, C_1}$};
    \node[h,rotate=90,minimum width=2cm] (h4) at (10,-2.5) {\small$h$};
    \node[bias,rotate=90,minimum width=2cm] (b4) at (11.25,-2.5) {\small$\text{bias}$};
    \node[fc,rotate=90,minimum width=2cm] (fc4) at (12.5,-2.5) {\small$\text{fc}_{Q, C_2}$};
  
    \node (rx) at (1.25,-2.5) {\small$\tilde{x}$};
  
    \draw[->] (x) -- (fc1);
    \draw[->] (fc1) -- (b1);
    \draw[->] (b1) -- (h1);
    \draw[->] (h1) -- (fc2);
    \draw[->] (fc2) -- (b2);
    \draw[->] (b2) -- (h2);
    \draw[->] (h2) -- (fc3);
    \draw[->] (fc3) -- (b3);
    \draw[->] (b3) -- (h3);
    \draw[-] (h3) -- (13.75,0);
    \draw[->] (13.75,0) -- (z);
    \draw[->] (z) -- (fc4);
    \draw[->] (fc4) -- (b4);
    \draw[->] (b4) -- (h4);
    \draw[->] (h4) -- (fc5);
    \draw[->] (fc5) -- (b5);
    \draw[->] (b5) -- (h5);
    \draw[->] (h5) -- (fc6);
    \draw[->] (fc6) -- (b6);
    \draw[->] (b6) -- (h6);
    \draw[->] (h6) -- (rx);

    \node[rotate=90] (L) at (1.25, -1.25) {\small$\mathcal{L}(\tilde{x}, x)$};
    \draw[-,dashed] (x) -- (L);
    \draw[-,dashed] (rx) -- (L);
  \end{tikzpicture}
  \vskip 6px
  \caption{A simple variant of a multi-layer perceptron based auto-encoder.
  Both encoder (top) and decoder (bottom) consist of 3-layer perceptrons
  taking an $R$-dimensional
  input $x$. The parameters $C_1, C_2,$ and $Q$ can be chosen; $Q$ also
  determines the size of the latent code $z$ and is usually chosen significantly
  lower than $R$ such that the auto-encoder learns a dimensionality reduction.
  The non-linearity $h$ is also not fixed and might be determined experimentally.
  The reconstruction loss $\mathcal{L}(\tilde{x}, x)$ quantifies the quality of
  the reconstruction $\tilde{x}$ and is minimized during training.}
  \label{subfig:deep-learning-auto-encoder}
\end{figure}

\begin{figure}
  \centering
  \begin{tikzpicture}
    \node (x) at (1.25,0) {\small$x$};
    
    %\node[noise,rotate=90,minimum width=3.3cm] (noise1) at(1.25,0) {\small$\text{noise}_{\sigma^2}$};
    \node[conv,rotate=90,minimum width=3.3cm] (conv1) at (2.5,0) {\small$\text{conv}_{1, C_1, K}$\,+\,$\text{bias}$};
    %\node[bias,rotate=90,minimum width=3cm] (bias1) at (3.75,0) {$\text{bias}$};
    \node[h,rotate=90,minimum width=3.3cm] (h1) at (3.75,0) {\small$h$};
    \node[pool,rotate=90,minimum width=3.3cm] (pool1) at (5,0) {\small$\text{pool}_{2}$};
    
    \node[conv,rotate=90,minimum width=3.3cm] (conv2) at (6.25,0) {\small$\text{conv}_{C_1, C_2, K}$\,+\,$\text{bias}$};
    %\node[bias,rotate=90,minimum width=3cm] (bias2) at (8.75,0) {$\text{bias}$};
    \node[h,rotate=90,minimum width=3.3cm] (h2) at (7.5,0) {\small$h$};
    \node[pool,rotate=90,minimum width=3.3cm] (pool2) at (8.75,0) {\small$\text{pool}_{2}$};
    \node[view,rotate=90,minimum width=3.3cm] (view2) at (10,0) {\small$\text{view}_{B, C_3}$};
    \node[fc,rotate=90,minimum width=3.3cm] (fc2) at (11.25,0) {\small$\text{fc}_{C_3,Q}$};
    
    \node (z) at (12.5,-3.75) {\small$z$};
    
    \node[h,rotate=90,minimum width=3.3cm] (h4) at (6.25,-3.75) {\small$h$};
    %\node[bias,rotate=90,minimum width=3cm] (bias4) at (8.75,-3.75) {$\text{bias}$};
    \node[conv,rotate=90,minimum width=3.3cm] (conv4) at (7.5,-3.75) {\small$\text{conv}_{C_2, C_1, K}$\,+\,$\text{bias}$};
    \node[up,rotate=90,minimum width=3.3cm] (up4) at (8.75,-3.75) {\small$\text{nnup}_{2}$};
    \node[view,rotate=90,minimum width=3.3cm] (view4) at (10,-3.75) {\small$\text{view}_{B, C_2, \frac{H}{4}, \frac{W}{4}, \frac{D}{4}}$};
    \node[fc,rotate=90,minimum width=3.3cm] (fc4) at (11.25,-3.75) {\small$\text{fc}_{Q,C_3}$};
    
    \node[h,rotate=90,minimum width=3.3cm] (h5) at (2.5,-3.75) {\small$h$};
    %\node[bias,rotate=90,minimum width=3cm] (bias5) at (3.75,-4) {$\text{bias}$};
    \node[conv,rotate=90,minimum width=3.3cm] (conv5) at (3.75,-3.75) {\small$\text{conv}_{C_2, 1, K}$\,+\,$\text{bias}$};
    \node[up,rotate=90,minimum width=3.3cm] (up5) at (5,-3.75) {\small$\text{nnup}_{2}$};
    
    \node (rx) at (1.25,-3.75) {\small$\tilde{x}$};
    
    %\draw[->] (x) -- (noise1);
    \draw[->] (x) -- (conv1);
    \draw[->] (conv1) -- (h1);
    %\draw[->] (bias1) -- (h1);
    \draw[->] (h1) -- (pool1);
    
    \draw[->] (pool1) -- (conv2);
    \draw[->] (conv2) -- (h2);
    %\draw[->] (bias2) -- (h2);
    \draw[->] (h2) -- (pool2);
    \draw[->] (pool2) -- (view2);
    \draw[->] (view2) -- (fc2);
    
    \draw[-] (fc2) -- (12.5,0);
    \draw[->] (12.5,0) -- (z);
    \draw[->] (z) -- (fc4);
    
    \draw[->] (fc4) -- (view4);
    \draw[->] (view4) -- (up4);
    \draw[->] (up4) -- (conv4);
    %\draw[->] (conv4) -- (bias4);
    \draw[->] (conv4) -- (h4);
    
    \draw[->] (h4) -- (up5);
    \draw[->] (up5) -- (conv5);
    \draw[->] (conv5) -- (h5);
    %\draw[->] (bias5) -- (h5);
    \draw[->] (h5) -- (rx);

    \node[rotate=90] (L) at (1.25, -1.875) {\small$\mathcal{L}(\tilde{x}, x)$};
    \draw[-,dashed] (x) -- (L);
    \draw[-,dashed] (rx) -- (L);
  \end{tikzpicture}
  \vskip 6px
  % TODO short caption
  \caption{Illustration of a convolutional auto-encoder consisting of encoder (top)
  and decoder (bottom). Both are modeled using two stages of convolutional
  layers each followed by a bias layer and a non-linearity layer. The encoder uses
  max pooling to decrease the spatial size of the input; the decoder uses upsampling
  to increase it again. The number of channels $C_1$, $C_2$ and $C_3$ as well as
  the size $Q$ are hyper parameters. We assume the input to comprise one channel.
  Again, the reconstruction loss $\mathcal{L}(\tilde{x}, x)$ quantifies the quality of
  the reconstruction and is minimized during training.}
  \label{fig:deep-learning-convolutional-auto-encoder}
\end{figure}

\begin{neuralnetwork}[height=4]
    \newcommand{\nodetextclear}[2]{}
    % use \ifnum to get different labels
    \newcommand{\nodetextx}[2]{\ifnum #2=4 $x_n$ \else $x_#2$ \fi}
    \newcommand{\nodetexty}[2]{$y_#2$}
    % use exclude to turn off drawing of specific layers
    \inputlayer[count=4, bias=false, exclude={3}, title=Input\\layer, text=\nodetextx]
    \hiddenlayer[count=3, bias=false, title=Hidden\\layer, text=\nodetextclear]
      \linklayers[not from={3}]
    \outputlayer[count=4, exclude={3}, title=Output\\layer, text=\nodetextx] 
      \linklayers[not to={3}]

    % draw dots
    \path (L0-2) -- node{$\vdots$} (L0-4);
    \path (L2-2) -- node{$\vdots$} (L2-4);
\end{neuralnetwork}


==> inputs/GWOclassical.tex <==


We assume that $P$ parameters should be estimated: $K^{1},K^{2}, \ldots,K^{i}, \ldots,  K^{P}$, where $P \geq 1$. The following notations will be used:\\
\noindent $\bullet$ $P$ is the number of expected parameters, which are indexed with $i$.\\
$\bullet$ ${\rm iter}$ denotes one iteration and ${\rm T_{max}}$ the maximum allowed number of iterations.\\
$\bullet$ $f(\cdot)$ is the function to be minimized, also called the criterion. It depends on the $P$ parameters mentioned above.\\
$\bullet$ $\xqK{\rm iter}$ is a vector corresponding to one search agent $q=1,\ldots,Q$, at iteration ${\rm iter}$. It takes the form of a vector with a $P$-tuple of tested values $\xqK{\rm iter}=\left[K^{1},K^{2}, \ldots, K^{P}\right]^{T}$.\\
The seminal \textit{GWO} searches a continuous space. Among the search agents, there are three leaders $\alpha$, $\beta$, and $\delta$. All other agents are the $\omega$ wolves.\\ 
$\bullet$ $\xK{\alpha}$, $\xK{\beta}$, and $\xK{\delta}$ denote the position (in the form of a $P$-dimensional vector) of the leaders $\alpha$, $\beta$, and $\delta$ respectively.\\  
The position of any $\omega$ wolf at iteration ${\rm iter+1}$ is calculated as:
\begin{equation}\label{eq:GWO_Xmethod}
\xqK{iter+1} = \frac{1}{3}(\textbf{y}_{\alpha} + \textbf{y}_{\beta} + \textbf{y}_{\delta})
\end{equation}
It results from the equal contribution of the $\alpha$, $\beta$, and $\delta$ wolves. These contributions are computed at each iteration ${\rm iter}$ as follows, for any leader $l$, either $\alpha$, $\beta$, or $\delta$: 
\begin{equation}
\textbf{y}_{l} = \xK{l} - \arA \circ \arD_{l}
\end{equation}
with: $\arD_{l} = |\arC \circ \xK{l} -  \xqK{iter}|$\\

% \textcolor{red}{A global version of the continuous GWO has been proposed in \cite{Martin_MarotAppliedSoftComputing_18}. It involves, in addition to the three leaders mentioned above, two leaders $\rho_{1}$ and $\rho_{2}$ selected randomly among the herd of wolves.
% The corresponding modified update rule is as follows:
% \begin{equation}\label{eq:GWO_Xmethodglobal}
% \xqK{iter+1} = \frac{1}{5}(\vectorcontributionleader{\alpha} + \vectorcontributionleader{\beta} + \vectorcontributionleader{\delta} +
% \vectorcontributionleader{\rho_{1}}+
% \vectorcontributionleader{\rho_{2}}
% )
% \end{equation}
% }

The vectors $\arA$ and $\arC$ are calculated as $\arA=2\ara \circ \arr_{1} -  \ara$ and $\arC=2 \arr_{2}$. In these expressions,
the components of vector $\ara$ are all equal to $a$, a scalar value which is a key parameter in the algorithm. The value of $a$ decreases from 2 to 0 during the iterations. Vectors $\arr_{1}$, $\arr_{2}$ have random components between 0 and 1.\\ 
For the $i^{\rm th}$ parameter:\\

The component $b^{i}$ of $\arA$ is provided by: 
\begin{equation}\label{Eq:bi}
b^{i}=2 a r_{1} - a, 
\end{equation}
the same whatever $i$.\\
The component $d_{l}^{i}$ of $\arD_{l}$ is provided by: 
\begin{equation}\label{Eq:dli}
d_{l}^{i}=|2 r_{2} \xdimi{l} - \xqi{i}{iter}|
\end{equation}

where :

\begin{itemize}
\item $r_{1}$ and $r_{2}$ are two random values between 0 and 1;
\item $\xqi{i}{iter}$ is the $i^{\rm th}$ component of the $q^{\rm th}$ agent at iteration ${\rm iter}$;
\item $\xdimi{l}$  is the $i^{\rm th}$ component of leader $l$.
\end{itemize}

The component $\ydimi{l}$ of $\textbf{y}_{l}$ is provided by: 

\begin{equation}\label{Eq:yli}
\ydimi{l} = \xdimi{l} - b^{i} d_{l}^{i}
\end{equation}


During the hunt, the wolves firstly diverge from each other to search for the prey, or equivalently to encircle it. Secondly, they converge to kill the prey. This is mathematically modeled through the deterministic vector $\ara$. When $a>1$, 
the search agents are obliged to diverge from the prey: this is the exploration phase. Conversely, when $a \leq 1$, the search agents are obliged to attack towards the prey: this is the exploitation phase. In the seminal version of \textit{GWO} \cite{Mirjalili201446}, the key parameter $a$ decreased regularly from 2 to 0: $a=2(1 - \frac{{\rm iter} }{T_{max}})$, where ${\rm iter}$ is the iteration index, and $T_{max}$ is the maximum number of iterations. In more recent works, various expressions have been proposed for $a$ such as a quadratic \cite{Mittal2016} or adaptive \cite{Martin_MarotAppliedSoftComputing_18} function. Whatever the version \cite{Mittal2016,Martin_MarotAppliedSoftComputing_18} the exploration phase lasts until $a=1$, then the exploitation phase lasts from $a=1$ to $a=0$.

==> inputs/PlotTestFunctions.tex <==


\begin{figure}[h!]
\centering{
 \begin{tabular}{c@{\,}c@{\,}}
  \includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF1.eps}
 &\includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF2.eps}\\
  \includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF3.eps}
 &\includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF4.eps}\\
  \includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF5.eps}&
   \end{tabular}
\caption{From left to right and top to bottom: Plots F1 to F5 centered on (1,0) \label{fig:testfunctionsF1to5} }}
\end{figure}

\begin{figure}[h!]
\centering{
 \begin{tabular}{c@{\,}c@{\,}}
  \includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF6.eps}
 &\includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF7.eps}\\
  \includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF8.eps}
 &\includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF9.eps}\\
  \includegraphics[width=4.0cm]{Figures/TestFunctions/PlotF10.eps}&
   \end{tabular}
\caption{From left to right and top to bottom: Plots F6 to F10 centered on (1,0) \label{fig:testfunctionsF6to10} }}
\end{figure}
  
